Derived category of the spinor 15-fold

We construct a full exceptional Lefschetz collection on the spinor 15-fold consisting of a connected component of the space of orthogonal 6-dimensional subspaces of a 12-dimensional complex vector space, isotropic with respect of a fixed non-degenerate quadratic form. The collection is made of 2 twists of a 4-item block and 8 twists of a 3-item block, confirming a conjecture of Kuznetsov and Smirnov. We speculate that a similar collection might work for the Freudenthal E7-variety.

==> python_script.tex <==
import numpy as np
import subprocess

# determinant bundle
def determinant(w):
    d=(2*w[0]+3*w[1]+4*w[2]+6*w[3]+5*w[4]+4*w[5]+3*w[6])/3
    return d

# ------------------------- ------------------------- ------------------------- #

# twist O(i)
def twist(w,i):
    wnew=np.array([w[0],w[1],w[2],w[3],w[4],w[5],w[6]+i]).astype(int)
    return wnew

# ------------------------- ------------------------- ------------------------- #

# twist O(i) for lists
def list_twist(list_w,i):
    list_wnew=[]
    for w in list_w:
        wnew=np.array([w[0],w[1],w[2],w[3],w[4],w[5],w[6]+i]).astype(int)
        list_wnew.append(wnew)
    return list_wnew


# ------------------------- ------------------------- ------------------------- #

# dual bundle
def dual(w):
    app=np.array([w[5],w[1],w[4],w[3],w[2],w[0],0])
    last_twist=int(np.around(-determinant(w)-determinant(app),decimals=5))
    d=np.array([w[5],w[1],w[4],w[3],w[2],w[0],last_twist]).astype(int)
    return d

# ------------------------- ------------------------- ------------------------- #

# dual bundle
def dual_direct_sum_bundles(list_w):
    list_d=[]
    for w in list_w:
        app=np.array([w[5],w[1],w[4],w[3],w[2],w[0],0])
        last_twist=int(np.around(-determinant(w)-determinant(app),decimals=5))
        d=np.array([w[5],w[1],w[4],w[3],w[2],w[0],last_twist]).astype(int)
        list_d.append(d)
    return list_d

# print(dual_direct_sum_bundles([np.array([1,0,0,0,0,0,0]),np.array([0,0,0,0,0,1,-2])]))


# ------------------------- ------------------------- ------------------------- #

# degree of cohomology by Bott for E7/P1
def cohomology_in_degree(coeffwro):
    
# I already have w + ro in the basis of wikipedia for E7
    w1=np.array([1,-1,0,0,0,0,0,0])
    w3=np.array([2,-1,-1,0,0,0,0,0])
    w4=np.array([3,-1,-1,-1,0,0,0,0])
    w5=np.array([9/4,-3/4,-3/4,-3/4,-3/4,1/4,1/4,1/4])
    w6=np.array([3/2,-1/2,-1/2,-1/2,-1/2,-1/2,1/2,1/2])
    w7=np.array([3/4,-1/4,-1/4,-1/4,-1/4,-1/4,-1/4,3/4])
    w2=np.array([7/4,-1/4,-1/4,-1/4,-1/4,-1/4,-1/4,-1/4])


    index=0
# check when (w + ro )(alpha)=0
    for i in range(1,8):
        for j in range(i+1,8):
            if (coeffwro[i]>coeffwro[j]): index=index+1
            if (coeffwro[i]==coeffwro[j]): 
                index=-100
                
    for i in range(1):
        for j in range(i+1,8):
            if (coeffwro[i]<coeffwro[j]): index=index+1
            if (coeffwro[i]==coeffwro[j]): 
                index=-100

    app=np.array([-1,-1,-1,-1,-1,-1,-1,-1])
    for i1 in range(1):
        app[i1]=1
        for i2 in range(i1+1,8):
            app[i2]=1
            for i3 in range(i2+1,8):
                app[i3]=1
                for i4 in range(i3+1,8):
                    app[i4]=1
                    if ( np.dot(coeffwro,app)<0 ): index=index+1
                    if ( np.dot(coeffwro,app)==0 ): 
                        index=-100
                    app[i4]=-1
                app[i3]=-1
            app[i2]=-1
        app[i1]=-1
    
    return index   
    
# ------------------------- ------------------------- ------------------------- #

# what is the cohomology group
def what_is_the_cohomology_group(wro):
# I already have w + ro in the basis of wikipedia for E7        
    w1=np.array([1,-1,0,0,0,0,0,0])
    w3=np.array([2,-1,-1,0,0,0,0,0])
    w4=np.array([3,-1,-1,-1,0,0,0,0])
    w5=np.array([9/4,-3/4,-3/4,-3/4,-3/4,1/4,1/4,1/4])
    w6=np.array([3/2,-1/2,-1/2,-1/2,-1/2,-1/2,1/2,1/2])
    w7=np.array([3/4,-1/4,-1/4,-1/4,-1/4,-1/4,-1/4,3/4])
    w2=np.array([7/4,-1/4,-1/4,-1/4,-1/4,-1/4,-1/4,-1/4])
    
    j=np.argmax(np.abs(wro))
    if (wro[j]<0): wro=-wro
    wro=np.sort(wro)
    wplusro=np.array([wro[7],wro[0],wro[1],wro[2],wro[3],wro[4],wro[5],wro[6]])
    coeffw=wplusro - w1-w2-w3-w4-w5-w6-w7
    w=np.array([-1,-1,-1,-1,-1,-1,-1,])
    w[0]=np.dot(coeffw,[0,-1,1,0,0,0,0,0])
    w[2]=np.dot(coeffw,[0,0,-1,1,0,0,0,0])
    w[3]=np.dot(coeffw,[0,0,0,-1,1,0,0,0])
    w[4]=np.dot(coeffw,[0,0,0,0,-1,1,0,0])
    w[5]=np.dot(coeffw,[0,0,0,0,0,-1,1,0])
    w[6]=np.dot(coeffw,[0,0,0,0,0,0,-1,1])
    w[1]=np.dot(coeffw,[0.5,0.5,0.5,0.5,-0.5,-0.5,-0.5,-0.5])
    w=w.astype(int)
    return w




def what_is_the_cohomology_group_correct(w):
    string_w = ",".join(map(str,w))
    p = subprocess.Popen(['/home/vbenedetti/Téléchargements/conLiE/LiE/Lie.exe'],
                     stdin=subprocess.PIPE,
                     stdout=subprocess.PIPE,
                     )
    cmd="dominant(["+string_w+"],E7)\n"
    p.stdin.write(cmd.encode());
    out=p.communicate()[0]
    p.stdin.close();
    p.wait();
    dom=out.decode().replace(" ","").replace("\n","")
    dom_w= np.fromstring(dom[1:-1], dtype=int, sep=',')
    dom_w=dom_w - np.array([1,1,1,1,1,1,1])
    
    return dom_w



# ------------------------- ------------------------- ------------------------- #



# Bott for E7(1)
def is_there_cohomology(w):
    
# the weight is w in Bourbaki's notation
# w + ro
    wro=w + np.array([1,1,1,1,1,1,1])

# w + ro in the basis of wikipedia for E7
    w1=np.array([1,-1,0,0,0,0,0,0])
    w3=np.array([2,-1,-1,0,0,0,0,0])
    w4=np.array([3,-1,-1,-1,0,0,0,0])
    w5=np.array([9/4,-3/4,-3/4,-3/4,-3/4,1/4,1/4,1/4])
    w6=np.array([3/2,-1/2,-1/2,-1/2,-1/2,-1/2,1/2,1/2])
    w7=np.array([3/4,-1/4,-1/4,-1/4,-1/4,-1/4,-1/4,3/4])
    w2=np.array([7/4,-1/4,-1/4,-1/4,-1/4,-1/4,-1/4,-1/4])

    coeffwro= wro[0]*w1+wro[1]*w2 + wro[2]*w3 + wro[3]*w4 + wro[4]*w5 + wro[5]*w6 + wro[6]*w7 
    # print(w, coeffwro, end = "")

    index=1
# check when (w + ro )(alpha)=0
    for i in range(8):
        for j in range(i+1,8):
            # because I had obscure problems with approximations, I had to add numpy.around
            if (np.around(coeffwro[i], decimals=5)==np.around(coeffwro[j], decimals=5)): 
                index=0

    app=np.array([1,1,1,1,1,1,1,1])
    for i1 in range(8):
        app[i1]=-1
        for i2 in range(i1+1,8):
            app[i2]=-1
            for i3 in range(i2+1,8):
                app[i3]=-1
                for i4 in range(i3+1,8):
                    app[i4]=-1
                    # because I had obscure problems with approximations, I had to add numpy.around
                    if ( np.around(np.dot(coeffwro,app), decimals=5)==0 ): 
                        index=0

                    app[i4]=1
                app[i3]=1
            app[i2]=1
        app[i1]=1
    
    deg=-1
    coh=np.array([-1,-1,-1,-1,-1,-1,-1])
    
    # if (index==1) : 
    #     deg=cohomology_in_degree(coeffwro)
    #     coh=what_is_the_cohomology_group(coeffwro)
        # print("  ===>>> ", "H^(", deg, ") = ", end = "")
        # print(coh, end = "")
    # print(" ")
    
    deg=cohomology_in_degree(coeffwro)
    coh=what_is_the_cohomology_group_correct(wro)
        # print("  ===>>> ", "H^(", deg, ") = ", end = "")
        # print(coh, end = "")
    # print(" ")
    index=0
    # print(coh)
    if (np.min(coh)>=0): index=1
        
    return index,deg,coh
    
        
# ------------------------- ------------------------- ------------------------- #


def print_cohomology_list(list_w):
    for w in list_w:
        index,deg,coh=is_there_cohomology(w)
        if (index==1): print("weight = ", w, " ====> H^", deg, " = ", coh)
            

# ------------------------- ------------------------- ------------------------- #


# dimension representation with LiE
def dimension_rep(w):
    # transform w in string to use lie
    string_w = ",".join(map(str,w))
    p = subprocess.Popen(['/home/vbenedetti/Téléchargements/conLiE/LiE/Lie.exe'],
                     stdin=subprocess.PIPE,
                     stdout=subprocess.PIPE,
                     )
    cmd="dim(["+string_w+"],E7)\n"
    p.stdin.write(cmd.encode());
    out=p.communicate()[0]
    p.stdin.close();
    p.wait();
    dim=int(out.decode().replace(" ","").replace("\n",""))
    return dim

# print(dimension_rep(np.array([0,0,0,0,0,0,1])))


# ------------------------- ------------------------- ------------------------- #


# basic tensor interface with LiE
def tensor_with_lie(string_w1,string_w2):
    p = subprocess.Popen(['/home/vbenedetti/Téléchargements/conLiE/LiE/Lie.exe'],
                     stdin=subprocess.PIPE,
                     stdout=subprocess.PIPE,
                     )
    cmd="tensor(["+string_w1+"],["+string_w2+"],E6)\n"
    p.stdin.write(cmd.encode());
    out=p.communicate()[0]
    p.stdin.close();
    p.wait();
    return out.decode()


# ------------------------- ------------------------- ------------------------- #


# tensor product of irreducible representations; returns array of weights 
def tensor(w1,w2):
    
    d=determinant(w1)+determinant(w2)
    
    # take only the E6 part of w1 and w2
    w1_E6=np.array([w1[0],w1[1],w1[2],w1[3],w1[4],w1[5]])
    w2_E6=np.array([w2[0],w2[1],w2[2],w2[3],w2[4],w2[5]])
    # transform w in string to use lie
    string_w1 = ",".join(map(str,w1_E6))
    string_w2 = ",".join(map(str,w2_E6))
    
    # use lie to produce the string of the tensor product
    string_tens = tensor_with_lie(string_w1,string_w2)
    
    # transform the string into a list of weights; if multiplicity is >1, weight appears more than once in the list
    string_tens=string_tens.replace(" ", "")
    string_tens=string_tens.replace("\n", "")
    sep=[s for s in string_tens.split('+')]
    # print(sep)   ======>   ['1X[0,0,0,0,0,0]', '1X[3,0,0,0,0,0]']
    tens_decomp=[]
    for pol in sep:
        mult_rep=[s for s in pol.split('X')]
        weight_E6=np.fromstring(mult_rep[1][1:-1], dtype=int, sep=',')
        last_twist= int(np.around(d-determinant(np.append(weight_E6,0)) ,decimals=5))
        weight = np.append(weight_E6,last_twist)
        for i in range(int(mult_rep[0])):
            tens_decomp.append(np.array([weight[0],weight[1],weight[2],weight[3],weight[4],weight[5],weight[6]]))
            
        
    return tens_decomp

# u=tensor(np.array([1,0,0,0,0,1,-4]), np.array([1,0,0,0,0,1,0]))
# print(u)


# ------------------------- ------------------------- ------------------------- #


def chi_direct_sum_bundles(list_weight):
    chi=0
    for w in list_weight:
        index,deg,coh = is_there_cohomology(w)
        if (index==1):
            chi=chi + ((-1)**deg)*dimension_rep(coh) 
            
    return chi
    
# chi_direct_sum_bundles([np.array([1,0,0,0,0,0,0]),np.array([0,0,0,0,0,1,-2])])


# ------------------------- ------------------------- ------------------------- #

def endomorphisms_direct_sum_bundles(list_weight):
    list_weight_dual=dual_direct_sum_bundles(list_weight)
    endo=[]
    for w in list_weight:
        for dw in list_weight_dual:
            tensor_temp=tensor(w,dw)
            for weight in tensor_temp:
                endo.append(weight)
    return endo

# print(endomorphisms_direct_sum_bundles([np.array([1,0,0,0,0,0,0]),np.array([0,0,0,0,0,1,-2])]))  

# ------------------------- ------------------------- ------------------------- #

def endomorphisms_with_twist(list_weight,i):
    list_weight_dual=dual_direct_sum_bundles(list_weight)
    endo=[]
    for w in list_weight:
        for dw in list_weight_dual:
            tensor_temp=tensor(w,dw)
            for weight in tensor_temp:
                endo.append(twist(weight,i))
    return endo

    
# ------------------------- ------------------------- ------------------------- #

def morphisms_direct_sum_bundles(list_weight1,list_weight2):
    list_weight_dual=dual_direct_sum_bundles(list_weight1)
    mor=[]
    for w in list_weight2:
        for dw in list_weight_dual:
            tensor_temp=tensor(w,dw)
            for weight in tensor_temp:
                mor.append(weight)
    return mor

# print(endomorphisms_direct_sum_bundles([np.array([1,0,0,0,0,0,0]),np.array([0,0,0,0,0,1,-2])]))    

    
# ------------------------- ------------------------- ------------------------- #


# search for a bundle such that chi(End)=id, chi(End(-1))=0, chi(End(-2))\neq 0

# variant programs for chi
# here the weights have 8 entries instead of 7; 
# the last entry is useful to tell the program in which shift the bundle lives

def chi_sequence(list_weight):
    chi=0
    for w in list_weight:
        index,deg,coh = is_there_cohomology(np.array([w[0],w[1],w[2],w[3],w[4],w[5],w[6]]))
        if (index==1):
            chi=chi + w[8]*((-1)**(np.abs(w[7])))*((-1)**deg)*dimension_rep(coh) 
            
    return chi


# ------------------------- ------------------------- ------------------------- #


def endo_twist_sequence(list_weight,i):
    list_weight_dual=dual_sequence(list_weight)
    endo=[]
    for w in list_weight:
        for dw in list_weight_dual:
            tensor_temp=tensor_E7T1(w,dw)
            for weight in tensor_temp:
                endo.append(twist_sequence(weight,i))
    return endo

    
# ------------------------- ------------------------- ------------------------- #

# twist O(i)
def twist_sequence(w,i):
    wnew=np.array([w[0],w[1],w[2],w[3],w[4],w[5],w[6]+i,w[7],w[8]]).astype(int)
    return wnew

# ------------------------- ------------------------- ------------------------- #


def dual_sequence(list_w):
    list_d=[]
    for w in list_w:
        app=np.array([w[5],w[1],w[4],w[3],w[2],w[0],0])
        last_twist=int(np.around(-determinant(np.array([w[0],w[1],w[2],w[3],w[4],w[5],w[6]]))-determinant(app) ,decimals=5))
        d=np.array([w[5],w[1],w[4],w[3],w[2],w[0],last_twist,-w[7],w[8]]).astype(int)
        list_d.append(d)
    return list_d


# ------------------------- ------------------------- ------------------------- #


# tensor product of irreducible representations; returns array of weights 
def tensor_E7T1(w1,w2):
    
    w1e=np.array([w1[0],w1[1],w1[2],w1[3],w1[4],w1[5],w1[6]])
    w2e=np.array([w2[0],w2[1],w2[2],w2[3],w2[4],w2[5],w2[6]])
    d=determinant(w1e)+determinant(w2e)
    
    # take only the E6T1 part of w1 and w2
    w1_E6T1=np.array([w1[0],w1[1],w1[2],w1[3],w1[4],w1[5],w1[7]])
    w2_E6T1=np.array([w2[0],w2[1],w2[2],w2[3],w2[4],w2[5],w2[7]])
    # transform w in string to use lie
    string_w1 = ",".join(map(str,w1_E6T1))
    string_w2 = ",".join(map(str,w2_E6T1))
    
    # use lie to produce the string of the tensor product
    string_tens = tensor_LiE_E6T1(string_w1,string_w2)
    
    # transform the string into a list of weights; if multiplicity is >1, weight appears more than once in the list
    string_tens=string_tens.replace(" ", "")
    string_tens=string_tens.replace("\n", "")
    sep=[s for s in string_tens.split('+')]
    # print(sep)   ======>   ['1X[0,0,0,0,0,0]', '1X[3,0,0,0,0,0]']
    
    tens_decomp=[]
    for pol in sep:
        mult_rep=[s for s in pol.split('X')]
        weight_E6=np.fromstring(mult_rep[1][1:-1], dtype=int, sep=',')
        
        last_twist= int(np.around(d-determinant(np.array(
            [weight_E6[0],weight_E6[1],weight_E6[2],weight_E6[3],weight_E6[4],weight_E6[5],0])) ,decimals=5))
        weight = np.append(weight_E6,last_twist)
        
        for i in range(int(mult_rep[0])):
            tens_decomp.append(np.array(
                [weight[0],weight[1],weight[2],weight[3],weight[4],weight[5],weight[7],weight[6], w1[8]*w2[8]]))
            
        
    return tens_decomp


# ------------------------- ------------------------- ------------------------- #


# basic tensor interface with LiE
def tensor_LiE_E6T1(string_w1,string_w2):
    p = subprocess.Popen(['/home/vbenedetti/Téléchargements/conLiE/LiE/Lie.exe'],
                     stdin=subprocess.PIPE,
                     stdout=subprocess.PIPE,
                     )
    cmd="tensor(["+string_w1+"],["+string_w2+"],E6T1)\n"
    p.stdin.write(cmd.encode());
    out=p.communicate()[0]
    p.stdin.close();
    p.wait();
    return out.decode()


# ------------------------- ------------------------- ------------------------- #


def morphisms_sequence(list_weight1,list_weight2):
    list_weight_dual=dual_sequence(list_weight1)
    mor=[]
    for w in list_weight2:
        for dw in list_weight_dual:
            tensor_temp=tensor_E7T1(w,dw)
            for weight in tensor_temp:
                mor.append(weight)
    return mor



# ------------------------- ------------------------- ------------------------- #

def check_twisted_endo_sequence(list_weight,i_max):
    for i in range(i_max):
        print("chi(End x O(-", i, ")) = ", chi_sequence(endo_twist_sequence(list_weight,-i)))
        

# ------------------------- ------------------------- ------------------------- #
        
        
def check_twisted_hom_sequence(list_weight1,list_weight2,i_max):
    for i in range(i_max):
        print("chi(Hom x O(-", i, ")) = ", chi_sequence(morphisms_sequence([w+i*O1 for w in list_weight1], list_weight2)) )


# ------------------------- ------------------------- ------------------------- #


def print_cohomology_sequence(list_w):
    for w in list_w:
        index,deg,coh=is_there_cohomology([w[0],w[1],w[2],w[3],w[4],w[5],w[6]])
        if (index==1): print("weight = ", w, " ====> H^", deg, " = ", coh)
            

# ------------------------- ------------------------- ------------------------- #


def cohomology_twisted_hom_sequence(list_weight1,list_weight2,i_min,i_max):
    for i in range(i_min,i_max):
        print(i)
        print_cohomology_sequence(morphisms_sequence([w+i*O1 for w in list_weight1], list_weight2)) 


# ------------------------- ------------------------- ------------------------- #









# ------------------------- ------------------------- ------------------------- #
# ------------------------- ------------------------- ------------------------- #
# ------------------------- ------------------------- ------------------------- #
# ------------------------- ------------------------- ------------------------- #
# ------------------------- ------------------------- ------------------------- #
# ------------------------- ------------------------- ------------------------- #
# ------------------------- ------------------------- ------------------------- #
# ------------------------- ------------------------- ------------------------- #
# ------------------------- ------------------------- ------------------------- #
# ------------------------- ------------------------- ------------------------- #
# ------------------------- ------------------------- ------------------------- #
# ------------------------- ------------------------- ------------------------- #
# ------------------------- ------------------------- ------------------------- #
# ------------------------- ------------------------- ------------------------- #
# ------------------------- ------------------------- ------------------------- #
# ------------------------- ------------------------- ------------------------- #
# ------------------------- ------------------------- ------------------------- #
# ------------------------- ------------------------- ------------------------- #
# ------------------------- ------------------------- ------------------------- #
# ------------------------- ------------------------- ------------------------- #
# ------------------------- ------------------------- ------------------------- #
# ------------------------- ------------------------- ------------------------- #
# ------------------------- ------------------------- ------------------------- #
# ------------------------- ------------------------- ------------------------- #
# ------------------------- ------------------------- ------------------------- #
# ------------------------- ------------------------- ------------------------- #
# ------------------------- ------------------------- ------------------------- #
# ------------------------- ------------------------- ------------------------- #
# ------------------------- ------------------------- ------------------------- #
# ------------------------- ------------------------- ------------------------- #
# ------------------------- ------------------------- ------------------------- #
# ------------------------- ------------------------- ------------------------- #
# ------------------------- ------------------------- ------------------------- #
# ------------------------- ------------------------- ------------------------- #
# ------------------------- ------------------------- ------------------------- #
# ------------------------- ------------------------- ------------------------- #
# ------------------------- ------------------------- ------------------------- #
# ------------------------- ------------------------- ------------------------- #
# ------------------------- ------------------------- ------------------------- #
# ------------------------- ------------------------- ------------------------- #
# ------------------------- ------------------------- ------------------------- #
# ------------------------- ------------------------- ------------------------- #
# ------------------------- ------------------------- ------------------------- #
# ------------------------- ------------------------- ------------------------- #
# ------------------------- ------------------------- ------------------------- #
# ------------------------- ------------------------- ------------------------- #
# ------------------------- ------------------------- ------------------------- #
# ------------------------- ------------------------- ------------------------- #
# ------------------------- ------------------------- ------------------------- #
# ------------------------- ------------------------- ------------------------- #
# ------------------------- ------------------------- ------------------------- #
# ------------------------- ------------------------- ------------------------- #
# ------------------------- ------------------------- ------------------------- #
# ------------------------- ------------------------- ------------------------- #
# ------------------------- ------------------------- ------------------------- #
# ------------------------- ------------------------- ------------------------- #
# ------------------------- ------------------------- ------------------------- #
# ------------------------- ------------------------- ------------------------- #
# ------------------------- ------------------------- ------------------------- #
# ------------------------- ------------------------- ------------------------- #
# ------------------------- ------------------------- ------------------------- #
# ------------------------- ------------------------- ------------------------- #
# ------------------------- ------------------------- ------------------------- #
# ------------------------- ------------------------- ------------------------- #
# ------------------------- ------------------------- ------------------------- #
# ------------------------- ------------------------- ------------------------- #
# ------------------------- ------------------------- ------------------------- #
# ------------------------- ------------------------- ------------------------- #
# ------------------------- ------------------------- ------------------------- #
# ------------------------- ------------------------- ------------------------- #
# ------------------------- ------------------------- ------------------------- #
# ------------------------- ------------------------- ------------------------- #




 


# from now on there will be only computations
# ------------------------- ------------------------- ------------------------- #
# ------------------------- ------------------------- ------------------------- #
# ------------------------- ------------------------- ------------------------- #
# ------------------------- ------------------------- ------------------------- #
# ------------------------- ------------------------- ------------------------- #
# ------------------------- ------------------------- ------------------------- #
# ------------------------- ------------------------- ------------------------- #
# ------------------------- ------------------------- ------------------------- #
# ------------------------- ------------------------- ------------------------- #
# ------------------------- ------------------------- ------------------------- #
# ------------------------- ------------------------- ------------------------- #
# ------------------------- ------------------------- ------------------------- #
# ------------------------- ------------------------- ------------------------- #
# ------------------------- ------------------------- ------------------------- #
# ------------------------- ------------------------- ------------------------- #
# ------------------------- ------------------------- ------------------------- #
# ------------------------- ------------------------- ------------------------- #
# ------------------------- ------------------------- ------------------------- #






# ------------------------- ------------------------- ------------------------- #
# ------------------------- ------------------------- ------------------------- #
# ------------------------- ------------------------- ------------------------- #
# let us verify the exceptional collection of length 3*18=54 with 0, O, P'

list_weight_o1=[np.array([0,0,0,0,0,0,0,0,1])]
list_weight_e1=[np.array([0,0,0,0,0,0,0,0,1]), np.array([1,0,0,0,0,0,0,0,1])]
list_weight_e2=[np.array([0,0,0,0,0,0,0,0,1]), np.array([1,0,0,0,0,0,0,0,1]), np.array([2,0,0,0,0,0,0,0,1])]


print("\nO1, E1,  E2, O1toE1, O1toE2, E1toE2\n")
for i in range(18):
    print(chi_direct_sum_bundles(endomorphisms_with_twist(list_weight_o1,-i)), "  ",
          chi_direct_sum_bundles(endomorphisms_with_twist(list_weight_e1,-i)), "  ",
          chi_direct_sum_bundles(endomorphisms_with_twist(list_weight_e2,-i)), "  ",
          chi_direct_sum_bundles(morphisms_direct_sum_bundles(list_twist(list_weight_e1,i),list_weight_o1)), "     ",
          chi_direct_sum_bundles(morphisms_direct_sum_bundles(list_twist(list_weight_e2,i),list_weight_o1)), "     ",
          chi_direct_sum_bundles(morphisms_direct_sum_bundles(list_twist(list_weight_e2,i),list_weight_e1))
         )
    
print("\n We obtain thus an exceptional collection of length 54!!")


# ------------------------- ------------------------- ------------------------- #
# result of computation above

O1, E1,  E2, O1toE1, O1toE2, E1toE2

1    1    1    0       0       0
0    0    0    0       0       0
0    0    0    0       0       0
0    0    0    0       0       0
0    0    0    0       0       0
0    0    0    0       0       0
0    0    0    0       0       0
0    0    0    0       0       0
0    0    0    0       0       0
0    0    0    0       0       0
0    0    0    0       0       0
0    0    0    0       0       0
0    0    0    0       0       0
0    0    0    0       0       0
0    0    0    0       0       0
0    0    0    0       0       0
0    0    0    0       0       0
0    0    0    0       0       0

 We obtain thus an exceptional collection of length 54!!



# ------------------------- ------------------------- ------------------------- #
# ------------------------- ------------------------- ------------------------- #
# ------------------------- ------------------------- ------------------------- #
#fet is the bundle Q' modulo some twist and left mutation (to be precise, Q'=L_{B',...,B'(4)}(fet(5)) ) in the paper; here we prove proposition 6.4

fet=[np.array([1,0,1,0,0,0,-5,0,1])
         ,np.array([2,0,0,0,0,0,-7,0,-1]),np.array([1,0,0,0,0,0,-7,0,-1]),np.array([0,0,0,0,0,0,-7,0,-1]) # -e2(-7)
         ,np.array([1,0,0,0,0,0,-6,0,112]),np.array([0,0,0,0,0,0,-6,0,112]) # e1(-6)
         ,np.array([2,0,0,0,0,0,-6,0,56]) # 56e2(-6)
         ,np.array([0,0,0,0,0,0,-5,0,-1673-3137+1]) # -1673e0(-5)
         ,np.array([1,0,0,0,0,0,-5,0,-3137+1]) # -3137e1(-5)
         ,np.array([2,0,0,0,0,0,-5,0,1]) # 1e2(-5)
         ,np.array([0,0,0,0,0,0,-4,0,94656-56]) # -94656e0(-4)
         ,np.array([1,0,0,0,0,0,-4,0,-56]) # 
         ,np.array([2,0,0,0,0,0,-4,0,-56]) # -56e2(-4)
         ,np.array([0,0,0,0,0,0,-3,0,-54342+3271-1]) # -54342e0(-3)
         ,np.array([1,0,0,0,0,0,-3,0,3271-1]) # 3271e1(-3)
         ,np.array([2,0,0,0,0,0,-3,0,-1]) # -1e2(-3)
         ,np.array([0,0,0,0,0,0,-2,0,-58576-968+56]) # -58576e0(-2)
         ,np.array([1,0,0,0,0,0,-2,0,-968+56]) # -968e1(-2)
         ,np.array([2,0,0,0,0,0,-2,0,56]) # 56e2(-2)
         ,np.array([0,0,0,0,0,0,-1,0,54342-3137]) # 54342e0(-1)
         ,np.array([1,0,0,0,0,0,-1,0,-3137]) # -3137e1(-1)
        ]

print("\n toO1, toE1, toE2\n")
for i in range(18):
    print(i,#chi_sequence(endo_twist_sequence(fet,-i)), "  ",
          chi_sequence(morphisms_sequence(list_weight_o1,fet-i*O1)), "     ",
          chi_sequence(morphisms_sequence(list_weight_e1,fet-i*O1)), "     ",
          chi_sequence(morphisms_sequence(list_weight_e2,fet-i*O1))
         )
    
for i in range(3):
    print(i,chi_sequence(endo_twist_sequence(fet,-i))
         )




# ------------------------- ------------------------- ------------------------- #
# result of computation above
toO1, toE1, toE2

0 0       0       0
1 0       0       0
2 0       0       0
3 0       0       0
4 0       0       0
5 0       0       0
6 0       0       0
7 0       0       0
8 0       0       0
9 0       0       0
10 0       0       0
11 0       0       0
12 0       0       0
13 0       0       0
14 0       0       0
15 0       0       0
16 0       0       0
17 0       0       0



0 1
1 0
2 -1



# ------------------------- ------------------------- ------------------------- #
# ------------------------- ------------------------- ------------------------- #
# ------------------------- ------------------------- ------------------------- #
#fet2 is the bundle L_{B'}Q'(1) modulo some twist and left mutation (to be precise, L_{B'}Q'=L_{B',...,B'(4)}(fet2(5)) ) in the paper; here we show that the residual collection Q',L_{B'}Q'(1)  is completely orthogonal (last computation)

fet2=[np.array([1,0,1,0,0,0,-4,0,1])
         ,np.array([2,0,0,0,0,0,-6,0,-1]),np.array([1,0,0,0,0,0,-6,0,-1]),np.array([0,0,0,0,0,0,-6,0,-1]) # -e2(-6)
         ,np.array([1,0,0,0,0,0,-5,0,112]),np.array([0,0,0,0,0,0,-5,0,112]) # e1(-5)
         ,np.array([2,0,0,0,0,0,-5,0,56]) # 56e2(-5)
         ,np.array([0,0,0,0,0,0,-4,0,-1673-3137+1]) # -1673e0(-4)
         ,np.array([1,0,0,0,0,0,-4,0,-3137+1]) # -3137e1(-4)
         ,np.array([2,0,0,0,0,0,-4,0,1]) # 1e2(-4)
         ,np.array([0,0,0,0,0,0,-3,0,94656-56]) # -94656e0(-3)
         ,np.array([1,0,0,0,0,0,-3,0,-56]) # 
         ,np.array([2,0,0,0,0,0,-3,0,-56]) # -56e2(-3)
         ,np.array([0,0,0,0,0,0,-2,0,-54342+3271-1]) # -54342e0(-2)
         ,np.array([1,0,0,0,0,0,-2,0,3271-1]) # 3271e1(-2)
         ,np.array([2,0,0,0,0,0,-2,0,-1]) # -1e2(-2)
         ,np.array([0,0,0,0,0,0,-1,0,-58576-968+56]) # -58576e0(-1)
         ,np.array([1,0,0,0,0,0,-1,0,-968+56]) # -968e1(-1)
         ,np.array([2,0,0,0,0,0,-1,0,56]) # 56e2(-1)
         ,np.array([0,0,0,0,0,0,0,0,54342-3137]) # 54342e0
         ,np.array([1,0,0,0,0,0,0,0,-3137]) # -3137e1
         
         ,np.array([1,0,0,0,0,0,0,1,-3136]) # -3136e1(1)
         ,np.array([0,0,0,0,0,0,0,0,-47936-3136]) # -47936e0(1)
        ]

print("\n toO1, toE1, toE2\n")
for i in range(18):
    print(i,#chi_sequence(endo_twist_sequence(fet,-i)), "  ",
          chi_sequence(morphisms_sequence(list_weight_o1,fet2-i*O1)), "     ",
          chi_sequence(morphisms_sequence(list_weight_e1,fet2-i*O1)), "     ",
          chi_sequence(morphisms_sequence(list_weight_e2,fet2-i*O1))
         )
    
print("\n BOOM!!!!!!!!!!!!!!!!!!!")

print(chi_sequence(endo_twist_sequence(fet,0)))
print(chi_sequence(endo_twist_sequence(fet,0)))
print(chi_sequence(morphisms_sequence(fet2,fet)))
print(chi_sequence(morphisms_sequence(fet,fet2)))


# ------------------------- ------------------------- ------------------------- #
# result of computation above

toO1, toE1, toE2

0 0       0       0
1 0       0       0
2 0       0       0
3 0       0       0
4 0       0       0
5 0       0       0
6 0       0       0
7 0       0       0
8 0       0       0
9 0       0       0
10 0       0       0
11 0       0       0
12 0       0       0
13 0       0       0
14 0       0       0
15 0       0       0
16 0       0       0
17 0       0       0

 BOOM!!!!!!!!!!!!!!!!!!!


1
1
0
0


# ------------------------- ------------------------- ------------------------- #
# ------------------------- ------------------------- ------------------------- #
# ------------------------- ------------------------- ------------------------- #
# this is the computation of the rectangular part of the collection whose terms are 0, O, P and their twists

list_weight_o1=[np.array([0,0,0,0,0,0,0,0,1])]
list_weight_e1=[np.array([0,0,0,0,0,0,0,0,1]), np.array([1,0,0,0,0,0,0,0,1])]
list_weight_e2=[np.array([0,0,1,0,0,0,-3,0,1])
                ,np.array([0,0,0,0,0,0,-3,0,-1+1])
                ,np.array([1,0,0,0,0,0,-3,0,1])
                ,np.array([0,0,0,0,0,0,-2,0,-56])
                ,np.array([1,0,0,0,0,0,-2,0,-56])
                ,np.array([0,0,0,0,0,0,-1,0,1597+133])
                ,np.array([1,0,0,0,0,0,-1,0,133])
                ,np.array([0,0,0,0,0,0,0,0,-7504])
               ]

    
print("\n BOOM!!!!!!!!!!!!!!!!!!!")

print("\n E2toE2     O1toE2 E1toE2\n")
for i in range(1,19):
    print(chi_sequence(morphisms_sequence(list_weight_e2+i*O1,list_weight_e2)), "  ", "  ", "  ", "  ",
          chi_sequence(morphisms_sequence(list_weight_o1+i*O1,list_weight_e2)), "     ",
          chi_sequence(morphisms_sequence(list_weight_e1+i*O1,list_weight_e2))
         )
for i in range(1):
    print(chi_sequence(morphisms_sequence(list_weight_e2+i*O1,list_weight_e2)), "  ", "  ", "  ", "  ",
          chi_sequence(morphisms_sequence(list_weight_e2+i*O1,list_weight_o1)), "     ",
          chi_sequence(morphisms_sequence(list_weight_e2+i*O1,list_weight_e1))
         )
    
print("\n We obtain thus an exceptional collection of length 54!!")



# ------------------------- ------------------------- ------------------------- #
# result of computation above

 BOOM!!!!!!!!!!!!!!!!!!!

 E2toE2     O1toE2 E1toE2

0             0       0
0             0       0
0             0       0
0             0       0
0             0       0
0             0       0
0             0       0
0             0       0
0             0       0
0             0       0
0             0       0
0             0       0
0             0       0
0             0       0
0             0       0
0             0       0
0             0       0
-1             0       0
1             0       0

 We obtain thus an exceptional collection of length 54!!



# ------------------------- ------------------------- ------------------------- #
# ------------------------- ------------------------- ------------------------- #
# ------------------------- ------------------------- ------------------------- #
#fett is the bundle L_{B}Q modulo some twist and left mutation (to be precise, L_{B}Q=L_{B,B(1),...,B(8)}(fett(8)) ) in the paper; here we prove proposition 6.5

fett=[np.array([1,0,1,0,0,0,-8,0,1])
         ,np.array([0,0,0,0,0,0,-8,0,-1])
         ,np.array([1,0,0,0,0,0,-8,0,-1])
         ,np.array([0,0,0,0,0,0,-7,0,112])
         ,np.array([1,0,0,0,0,0,-7,0,112])
         ,np.array([0,0,0,0,0,0,-6,0,-3270-3135])
         ,np.array([1,0,0,0,0,0,-6,0,-3135])
         ,np.array([0,0,0,0,0,0,-5,0,125512+6424])
         ,np.array([1,0,0,0,0,0,-5,0,6424])
         ,np.array([0,0,1,0,0,0,-3-5,0,1]),np.array([0,0,0,0,0,0,-3-5,0,-1+1]),np.array([1,0,0,0,0,0,-3-5,0,1]),np.array([0,0,0,0,0,0,-2-5,0,-56]),np.array([1,0,0,0,0,0,-2-5,0,-56]),np.array([0,0,0,0,0,0,-1-5,0,1597+133]),np.array([1,0,0,0,0,0,-1-5,0,133]),np.array([0,0,0,0,0,0,-5,0,-7504])
         ,np.array([0,0,0,0,0,0,-4,0,-416954+3269])
         ,np.array([1,0,0,0,0,0,-4,0,3269])
         ,np.array([0,0,1,0,0,0,-3-4,0,-1*56]),np.array([0,0,0,0,0,0,-3-4,0,-1+1]),np.array([1,0,0,0,0,0,-3-4,0,-1*56]),np.array([0,0,0,0,0,0,-2-4,0,+56*56]),np.array([1,0,0,0,0,0,-2-4,0,56*56]),np.array([0,0,0,0,0,0,-1-4,0,-(1597+133)*56]),np.array([1,0,0,0,0,0,-1-4,0,-133*56]),np.array([0,0,0,0,0,0,-4,0,7504*56])
         ,np.array([0,0,0,0,0,0,-3,0,-126480-6480])
         ,np.array([1,0,0,0,0,0,-3,0,-6480])
         ,np.array([0,0,1,0,0,0,-3-3,0,-1]),np.array([0,0,0,0,0,0,-3-3,0,-1+1]),np.array([1,0,0,0,0,0,-3-3,0,-1]),np.array([0,0,0,0,0,0,-2-3,0,56]),np.array([1,0,0,0,0,0,-2-3,0,56]),np.array([0,0,0,0,0,0,-1-3,0,-1597-133]),np.array([1,0,0,0,0,0,-1-3,0,-133]),np.array([0,0,0,0,0,0,-3,0,7504])
         ,np.array([0,0,0,0,0,0,-2,0,418761-3270])
         ,np.array([1,0,0,0,0,0,-2,0,-3270])
         ,np.array([0,0,1,0,0,0,-3-2,0,1*56]),np.array([0,0,0,0,0,0,-3-2,0,-1+1]),np.array([1,0,0,0,0,0,-3-2,0,1*56]),np.array([0,0,0,0,0,0,-2-2,0,-56*56]),np.array([1,0,0,0,0,0,-2-2,0,-56*56]),np.array([0,0,0,0,0,0,-1-2,0,(1597+133)*56]),np.array([1,0,0,0,0,0,-1-2,0,133*56]),np.array([0,0,0,0,0,0,-2,0,-7504*56])
         ,np.array([0,0,0,0,0,0,-1,0,125512+6536])
         ,np.array([1,0,0,0,0,0,-1,0,6536])
         ,np.array([0,0,1,0,0,0,-3-1,0,1]),np.array([0,0,0,0,0,0,-3-1,0,-1+1]),np.array([1,0,0,0,0,0,-3-1,0,1]),np.array([0,0,0,0,0,0,-2-1,0,-56]),np.array([1,0,0,0,0,0,-2-1,0,-56]),np.array([0,0,0,0,0,0,-1-1,0,1597+133]),np.array([1,0,0,0,0,0,-1-1,0,133]),np.array([0,0,0,0,0,0,-1,0,-7504])
         ,np.array([0,0,0,0,0,0,0,0,-420224+3136])
         ,np.array([1,0,0,0,0,0,0,0,3136])
         ,np.array([0,0,1,0,0,0,-3,0,-1*56]),np.array([0,0,0,0,0,0,-3,0,-1+1]),np.array([1,0,0,0,0,0,-3,0,-1*56]),np.array([0,0,0,0,0,0,-2,0,56*56]),np.array([1,0,0,0,0,0,-2,0,56*56]),np.array([0,0,0,0,0,0,-1,0,-(1597+133)*56]),np.array([1,0,0,0,0,0,-1,0,-133*56]),np.array([0,0,0,0,0,0,0,0,7504*56])
        ]

print("\n toO1, toE1, toE2\n")
for i in range(1,19):
    print(i,#chi_sequence(endo_twist_sequence(fett,-i)), "  ",
          chi_sequence(morphisms_sequence(list_weight_o1,fett-i*O1)), "     ",
          chi_sequence(morphisms_sequence(list_weight_e1,fett-i*O1)), "     ",
          chi_sequence(morphisms_sequence(list_weight_e2,fett-i*O1))
         )
    
print("\n BOOM!!!!!!!!!!!!!!!!!!!")

print(chi_sequence(endo_twist_sequence(fett,0)))
print(chi_sequence(endo_twist_sequence(fett,-1)))
print(chi_sequence(endo_twist_sequence(fett,-2)))



# ------------------------- ------------------------- ------------------------- #
# result of computation above

1 0       0       0
2 0       0       0
3 0       0       0
4 0       0       0
5 0       0       0
6 0       0       0
7 0       0       0
8 0       0       0
9 0       0       0
10 0       0       0
11 0       0       0
12 0       0       0
13 0       0       0
14 0       0       0
15 0       0       0
16 0       0       0
17 0       0       0
18 0       0       0

 BOOM!!!!!!!!!!!!!!!!!!!
 
 1
 0
 -1


# ------------------------- ------------------------- ------------------------- #
# ------------------------- ------------------------- ------------------------- #
# ------------------------- ------------------------- ------------------------- #
#fet is now the bundle L_{B,B(1)}Q(1) modulo some twist and left mutation (to be precise, L_{B,B(1)}Q(1)=L_{B,B(1),...,B(8)}(fet(9)) ) in the paper; here we show that the residual collection Q,L_{B}Q(1)  is completely orthogonal (last computation)

fet2=fett-O1
fet=[np.array([1,0,1,0,0,0,-8,0,1])
         ,np.array([0,0,0,0,0,0,-8,0,-1])
         ,np.array([1,0,0,0,0,0,-8,0,-1])
         ,np.array([0,0,0,0,0,0,-7,0,112])
         ,np.array([1,0,0,0,0,0,-7,0,112])
         ,np.array([0,0,0,0,0,0,-6,0,-3270-3135])
         ,np.array([1,0,0,0,0,0,-6,0,-3135])
         ,np.array([0,0,0,0,0,0,-5,0,125512+6424])
         ,np.array([1,0,0,0,0,0,-5,0,6424])
         ,np.array([0,0,1,0,0,0,-3-5,0,1]),np.array([0,0,0,0,0,0,-3-5,0,-1+1]),np.array([1,0,0,0,0,0,-3-5,0,1]),np.array([0,0,0,0,0,0,-2-5,0,-56]),np.array([1,0,0,0,0,0,-2-5,0,-56]),np.array([0,0,0,0,0,0,-1-5,0,1597+133]),np.array([1,0,0,0,0,0,-1-5,0,133]),np.array([0,0,0,0,0,0,-5,0,-7504])
         ,np.array([0,0,0,0,0,0,-4,0,-416954+3269])
         ,np.array([1,0,0,0,0,0,-4,0,3269])
         ,np.array([0,0,1,0,0,0,-3-4,0,-1*56]),np.array([0,0,0,0,0,0,-3-4,0,-1+1]),np.array([1,0,0,0,0,0,-3-4,0,-1*56]),np.array([0,0,0,0,0,0,-2-4,0,+56*56]),np.array([1,0,0,0,0,0,-2-4,0,56*56]),np.array([0,0,0,0,0,0,-1-4,0,-(1597+133)*56]),np.array([1,0,0,0,0,0,-1-4,0,-133*56]),np.array([0,0,0,0,0,0,-4,0,7504*56])
         ,np.array([0,0,0,0,0,0,-3,0,-126480-6480])
         ,np.array([1,0,0,0,0,0,-3,0,-6480])
         ,np.array([0,0,1,0,0,0,-3-3,0,-1]),np.array([0,0,0,0,0,0,-3-3,0,-1+1]),np.array([1,0,0,0,0,0,-3-3,0,-1]),np.array([0,0,0,0,0,0,-2-3,0,56]),np.array([1,0,0,0,0,0,-2-3,0,56]),np.array([0,0,0,0,0,0,-1-3,0,-1597-133]),np.array([1,0,0,0,0,0,-1-3,0,-133]),np.array([0,0,0,0,0,0,-3,0,7504])
         ,np.array([0,0,0,0,0,0,-2,0,418761-3270])
         ,np.array([1,0,0,0,0,0,-2,0,-3270])
         ,np.array([0,0,1,0,0,0,-3-2,0,1*56]),np.array([0,0,0,0,0,0,-3-2,0,-1+1]),np.array([1,0,0,0,0,0,-3-2,0,1*56]),np.array([0,0,0,0,0,0,-2-2,0,-56*56]),np.array([1,0,0,0,0,0,-2-2,0,-56*56]),np.array([0,0,0,0,0,0,-1-2,0,(1597+133)*56]),np.array([1,0,0,0,0,0,-1-2,0,133*56]),np.array([0,0,0,0,0,0,-2,0,-7504*56])
         ,np.array([0,0,0,0,0,0,-1,0,125512+6536])
         ,np.array([1,0,0,0,0,0,-1,0,6536])
         ,np.array([0,0,1,0,0,0,-3-1,0,1]),np.array([0,0,0,0,0,0,-3-1,0,-1+1]),np.array([1,0,0,0,0,0,-3-1,0,1]),np.array([0,0,0,0,0,0,-2-1,0,-56]),np.array([1,0,0,0,0,0,-2-1,0,-56]),np.array([0,0,0,0,0,0,-1-1,0,1597+133]),np.array([1,0,0,0,0,0,-1-1,0,133]),np.array([0,0,0,0,0,0,-1,0,-7504])
        ]


print(chi_sequence(endo_twist_sequence(fet2,0)))
print(chi_sequence(morphisms_sequence(fet2,fet)))
print(chi_sequence(morphisms_sequence(fet,fet2)))


# ------------------------- ------------------------- ------------------------- #
# result of computation above

1
0
0


















